An Introduction to Gaussian Process Models

Within the past two decades, Gaussian process regression has been increasingly used for modeling dynamical systems due to some beneficial properties such as the bias variance trade-off and the strong connection to Bayesian mathematics. As data-driven method, a Gaussian process is a powerful tool for nonlinear function regression without the need of much prior knowledge. In contrast to most of the other techniques, Gaussian Process modeling provides not only a mean prediction but also a measure for the model fidelity. In this article, we give an introduction to Gaussian processes and its usage in regression tasks of dynamical systems. Try Gaussian process regression yourself: https://gpr.tbeckers.com

==> inputs/acronyms.tex <==
\begin{acronym}[MIMO] %put longest acronym in the brackets
	\acro{I/O}{input/output}
	\acro{ISS}{input-to-state stable}
	\acro{BIBO}{bounded-input bounded-output}
	
	\acro{SISO}{single-input single-output}
	\acro{MISO}{multi-input single-output}
	\acro{SIMO}{single-input multi-output}
	\acro{MIMO}{multi-input multi-output}
	
	\acro{MPC}{model-predictive control}
	\acro{CBF}{control barrier function}
	\acro{CLF}{control Lyapunov function}
\end{acronym}

